Cloth Funnels: Canonicalized-Alignment for Multi-Purpose Garment Manipulation

Automating garment manipulation is challenging due to extremely high variability in object configurations. To reduce this intrinsic variation, we introduce the task of "canonicalized-alignment" that simplifies downstream applications by reducing the possible garment configurations. This task can be considered as "cloth state funnel" that manipulates arbitrarily configured clothing items into a predefined deformable configuration (i.e. canonicalization) at an appropriate rigid pose (i.e. alignment). In the end, the cloth items will result in a compact set of structured and highly visible configurations - which are desirable for downstream manipulation skills. To enable this task, we propose a novel canonicalized-alignment objective that effectively guides learning to avoid adverse local minima during learning. Using this objective, we learn a multi-arm, multi-primitive policy that strategically chooses between dynamic flings and quasi-static pick and place actions to achieve efficient canonicalized-alignment. We evaluate this approach on a real-world ironing and folding system that relies on this learned policy as the common first step. Empirically, we demonstrate that our task-agnostic canonicalized-alignment can enable even simple manually-designed policies to work well where they were previously inadequate, thus bridging the gap between automated non-deformable manufacturing and deformable manipulation. Code and qualitative visualizations are available at https://clothfunnels.cs.columbia.edu/. Video can be found at https://www.youtube.com/watch?v=TkUn0b7mbj0.

==> text/intro_v2.tex <==
\section{Introduction}




% NOTE: we can motivate usefulness of rigid goal conditioning with kinematic constraints. canonicalization should be task agnostic, but different downstream task-specific manipulation policies needs to interact with different parts of the cloth. E.g. folding shirt arms in v.s. folding shirt horizontally
% To motivate this properly, we need to give examples where the same shirt instance requires different rigid goals depending on downstream tasks.

% Getting stuck in local minima of writing. Going back to writing notes and 
% chain of thought brain dump mode: 
Why is everyday cloth manipulation conceptually simple for humans?
To us, there are only a few meaningful states shirts could

% VERSION 2.2
% COMMENT: It's quite hard to motivate this in a sexy manner.
% WHAT I DO LIKE IS "funnel", "task agnostic v.s. task-specific"
In-the-wild cloth manipulation is made easy if the cloth is setup mindful of the downstream manipulation.
Concretely, this involves canonicalizing the garment, which unfolds the garment into a standard configuration thus exposing all keypoints, while ensuring the downstream task manipulation can kinematically reach task-relevant parts of the cloth.
Rigid-goal conditioned canonicalizing are a fundamental skill for robotic cloth manipulation systems, because this task-agnostic skill \emph{funnels} severely self-occluded and crumpled garment configurations found in-the-wild into highly structured configurations, allowing for simple task-specific policies to predictably and robustly manipulate the garments.



\iffalse
    % VERSION 2.1
    % COMMENT: want to also emphasize rigid goal condition. This paragraph feels too much emphasis on canonicalization
    % missing a high level general introduction sentence
    Consider how we go through clothes pile after laundry.
    % too lengthy. go more to the point: task-agnostic canonicalization enables simple task-specific routines to robustly and predictably manipulation the garments. however, since different tasks manipulates different  
    One-by-one, we would align the garments at a specific pose, with a large swing then a small adjustment or two, before executing a routine folding algorithm.
    All the severely self-occluded and crumple states clothes could assume are turned into a standard configuration.
    This task-agnostic canonicalization step enables simple (i.e., hardcoded) task-specific routines to robustly and predictably manipulate the garments.
    % 

    % VERSION 2.0
    % COMMENT: feeling like canonicalization is what should be emphasize
    % MOTIVATING EXAMPLE 
    In-the-wild cloth manipulation is made easy through canonicalization:
    % in the wild a.k.a starting from crumpled initial states. Is this clear from in-the-wild or we need to be more specific?
    by first bringing severely self-occluded crumpled garments into their standard canonical configuration [at a specific pose], downstream tasks such as ironing and folding becomes easy.

    % SOME NOTES IN PREPARATION FOR VERSION 2.0
    Every day cloth manipulation
    effortlessly
    because conceptually involves only two different modes,
    first is canonicalizing garment into a standard state from the infinite number of configs
    then downstream cloth manipulation relies on highly regular repeatable actions (e.g. a folding algorithm).

    From these observations, we ask the following question:
    ``How can we define a unified learning framework over multiple primitives and cloths''


\fi

Many prior works have designed
While prior works have tackled visual goal conditioned manipulation, we argue their problem formulation is too general for typical cloth manipulation tasks.
Our key observation is goal-conditioned cloth manipulation is much simpler from a canonical state, given

In summary, our approach has three main contributions:
\begin{enumerate}
    \item \textbf{A canonicalization objective factorization}, which not only give a better landscape for learning and greedy interaction policies\footnote{don't like this word, too vague, also need to back up by experiments later.} but also enables rigid goal-conditioning (i.e., SE2 transforms) of the canonical pose by design.
    \item \textbf{A multi-primitive, multi-arm setup for canonicalization}, which enables efficient unfolding using high velocity flings while reliably reaching garments' canonical configurations with high precision\footnote{high precision means different things in different contexts, ideally swap out for something else} pick and places.
    \item \textbf{A real-world shirt ironing and folding system}, which demonstrates our key observation that cloth manipulation in the wild is made tractable given a robust and efficient rigid-goal conditioned canonicalization.
\end{enumerate}
<<<<<<< HEAD



% WHAT ARE CHALLENGES? SPECIFICALLY IN THIS CASE?
% Human cloth manipulation contains multiple modes of interaction which trades of speed and precision (\eg fast but inaccurate flings, small but precise adjustments).

==> text/intro_v3.tex <==
\section{Introduction}

% NOTE to Cheng, Shuran, and Alper: we have been refering to downstream simple hardcoded manipulation policies as ``state machines'', etc. I want to change it to a manufacturing industry standard word. Please help me find such a word.
% It would be really nice if we can come up with a better word, that fuses both canonicalization and alignment. I don't like rigid goal conditioning. 
% Should we call it CanAl?...

Why hasn't the garments manufacturing received the same level of success in automation as robotic manufacturing in other industries?
Due to cloths' infinite degrees of freedom, severe self-occlusion, and the possible crumpled states they can assume during many manufacturing stages, defining simple, repetitive controllers with low failure rates (which characterizes non-deformable manufacturing pipelines) is a challenging feat.
In this work, we ask: ``how \emph{should} category-level cloth manipulation pipelines be designed, which enables maximum flexibility to arbitrary initial configurations (\ie crumpled initial states) and manipulation task?''

% only discuss `real world' == don't consider approaches which fail to generalize to real
Recently, real-world cloth manipulation has received a lot of attention.
% state machines. don't generalize, but is effective for each task if its rigid assumptions on configuration is satisfied.
Some of the earliest cloth manipulation works designed elaborate state machines for core cloth manipulation tasks in manufacturing, such as cloth smoothing~\cite{ken2022speedfolding} and folding~\cite{zhou2021folding}, but only for a specific instance, configuration, and task.
% self-supervised approaches don't generalize to novel cloth instances or tasks
More recently, fully self-supervised approaches learn to unfold~\cite{ha2021flingbot} and tackle visual goal-conditioned manipulation of a single cloth instance~\cite{lee2020learning} from arbitrary initial configurations.
% collecting human annotations for every new task is costly
On the other hand, approaches which uses human demonstrations for smoothing~\cite{ken2022speedfolding}, folding~\cite{zhou2021folding}, but require costly human demonstrations/annotations.


% Key idea 
Our main observation is that if given appropriately-aligned and canonicalized garments and a garment category-level keypoint detector, keypoint-based cloth-manipulation state machines are sufficient for many manufacturing pipelines.
In other words, instead of learning arbitrary cloth manipulation tasks from arbitrary initial configurations, we hypothesize that it is sufficient to learn a robust canonicalization and alignment policy.
This is because it \emph{funnels} unstructured and self-occluded cloth configurations into highly structured states with clearly visible keypoints, enabling simple heuristics to work with high success rate.
%%% NOTE: we can motivate our rigid goal conditioning with manufacturing. Prior works that do visual goal condition or behaviour cloning is ill-suited for different manufacturing pipelines, like ironing (require garments in specific pose), embroider, simple sewing lines, etc.

We argue that learning a robust, task-agnostic, garment-category level canonicalization and alignment policy is an enabler for simple downstream task-specific state machines.
To this end, we propose a canonicalization and alignment objective, which factorizes into two terms, one which accounts for the deformation cost and another for the planar rigid transform cost of the garment.
We demonstrate that this objective function enables better canonicalization and alignment compared to a naive unfactorized per-vertex cost objective function.
We implement a self-supervised multi-primitive, dual-arm system for efficient unfolding using high velocity flings and fine-grained adjustments using quasi-static pick and places.
We directly deploy our simulation-trained policy in the real world, where we demonstrate its effectiveness in a steam-ironing and folding pipeline.
These downstream applications exploit the highly structured configurations from our policy 

In summary, our approach has three main contributions:
\begin{enumerate}
    % this first contribution is currently vague and requires revisiting after we have experiments actually investigating why reward works.
    \item \textbf{A canonicalization and alignment objective factorization}, which we show emperically correlates better with downstream cloth manipulation success.
    \item \textbf{A multi-primitive, multi-arm setup for canonicalization and alignment}, which uses dynamic flings and quasi-static pick \& places.
    \item \textbf{A real-world shirt steam-ironing and folding system}, which demonstrates our key observation that garment-category level cloth manipulation from arbitrary initial states is made tractable given a robust canonicalization and alignment.
\end{enumerate}

==> text/intro_v4.tex <==
\section{Introduction}

Why has garment manipulation proved more difficult to automate than more typical rigid and articulated objects? We argue that two key factors are severe self-occlusion, which is present in the large set of possible crumpled states, and the infinite degrees of freedom inherent to clothing. As a result, it is impractical to manually define manipulation policies which result in reliable manipulation — a cornerstone of current automated non-deformable manufacturing pipelines.

In this work, we explore bridging the gap between existing approaches to automation and the challenging domain of clothing. We show that when a robot first learns to robustly manipulate arbitrarily configured clothing items into a specific pose, downstream manipulation skills can be made to work significantly more reliably on deformable clothing.



% only discuss `real world' == don't consider approaches that fail to generalize to real
Recently, real-world cloth manipulation has received significant attention.
% state machines. don't generalize, but is effective for each task if its rigid assumptions on configuration are satisfied.
\todo{need to cite earlier works, like Peiter Abbeel's folding with  PR2}Some of the earliest cloth manipulation work employed elaborate state machines for core cloth manipulation tasks in manufacturing, such as cloth smoothing~\cite{ken2022speedfolding} and folding~\cite{zhou2021folding}, but only for a specific clothing instance, configuration, and task.
% self-supervised approaches don't generalize to novel cloth instances or tasks

More recently, learning-based approaches have shown success in creating more general cloth manipulation behavior. One such approach consists of supervised methods that use human demonstrations for smoothing~\cite{ken2022speedfolding} and folding~\cite{zhou2021folding} behaviors but require costly human demonstrations/annotations. Another recent line of work employs fully self-supervised learning and has shown success in learning to unfold~\cite{ha2021flingbot} and in tackling visual goal-conditioned manipulation of a single cloth instance~\cite{lee2020learning} from arbitrary initial configurations.
% collecting human annotations for every new task is costly


% Key idea 
Our main observation is that if given appropriately-aligned and canonicalized garments\todo{should define this, first time use the term}, keypoint-based task-specific state machines are sufficient for many garment manipulation tasks.
Instead of learning arbitrary cloth manipulation tasks from arbitrary initial configurations, we hypothesize that it is sufficient to learn a robust canonicalization and alignment policy from which other manipulation skills may be chained. This is because such a policy \emph{funnels} unstructured and self-occluded cloth configurations into highly structured states with clearly visible key points, enabling simple heuristics to work with a high success rate.

To this end, we define a new ``canonicalized-alignment'' task for garment manipulation, where the goal is to transform a garment from its arbitrary initial state into a canonical shape (defined by its category) and align it with a particular rigid pose defined by rotation and translation in a 2D plane.

The end result is a decomposition of garment manipulation into two factorized pieces. The first of which funnels a chaotic and diverse set of cloth configurations into a narrow distribution in a structured region of state space while the second piece consists of downstream behaviors that are able to rely on friendly initial configurations and high observability.




\todo{feels redundant}Enabled by canonicalized-alignment, we propose \textbf{CASSIE}, a recipe for multi-purpose garment manipulation, which includes \underline{c}anonicalization, \underline{a}lignment, and \underline{s}tate machines.
By learning to canonicalize, our approach can turn arbitrarily crumpled initial configurations into standard configurations where all the garment's key-points are visible.
By simultaneously learning alignment, the canonicalized garment can be appropriately positioned and oriented for the downstream state machine's kinematic constraints.
Lastly, by using a mature off-the-shelf key-point detector to extract a key-point garment representation, our proposed recipe enables the usage of key-point-based task-specific state machines.


\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figures/teaser.png} \vspace{-4mm}
    \caption{Transformed-canonicalization funnels a wide distribution of possible initial configurations into a small set of well structured and highly observable states.} \vspace{-5mm}
    \label{fig:task}
\end{figure}

Our primary contribution is the introduction of the ``canonicalized-alignment'' task for garment manipulation, which can be serve as \textit{universal} starting point for many downstream garment manipulation applications. To achieve this, we propose a learned multi-arm, multi-primitive manipulation policy that strategically choose between dynamic flings and quasi-static pick\&place actions to efficiently and precisely transform the garment into its canonicalized and aligned configuration. 
This policy is based on a novel factorized objective function that effectively guided the learning and avoid ambiguities and local minima which plague the generic goal-reaching formulations by decoupling shape and pose.
We evaluate our approach's effectiveness by applying CASSIE to multiple downstream garment manipulation tasks in the real-world on a physical robot, including category-level garment folding and ironing and we show empirically that incorporation of canonicalized-alignment significantly improves the reliability of downstream tasks. These results suggest that robust canonicalized-alignment provides a practical step forward toward general-purpose garment manipulation from arbitrary states for diverse tasks by significantly reducing the difficulty of learning performant downstream manipulation behavior.

==> text/introduction.tex <==
\section{Introduction}
%If robots are to enter our homes one day, they will inevitably have to learn how to fold laundry. Typical cloth manipulation works assume an initial state of a perfectly unfolded and aligned cloth. Before we as humans can start folding laundry, however, we first have to pull a cloth from a pile, unfold it to discover its parts, and align it on a surface. For example, if the cloth is a T-shirt, we first have to unfold the body and bring it to a T-shape position, which we refer to as the \emph{canonical pose}.

% If robots are to achieve general-purpose manipulation capabilities, they inevitably need to learn how to interact with deformable objects in many scenarios.

\alper{I'm struggling to begin this introduction}

Unfolding and folding laundry, aligning sheets of carbon-fiber on a mold at a factory, and positioning  sheets on a person during a surgical operation are only some of the tasks that require goal conditioned cloth manipulation.

\alper{Big jump but I do want to mention this before introducing it in challenges}
Although many prior works have studied folding of wearable garments, most of them make the assumption that the cloth begins in a perfectly \textit{canonicalized}\cite{huang2022mesh} state. In reality, clothes in natural environments are crumpled and self-occluded. What's the point of having a robot fold your clothes if you have to flatten them first? 

Despite the importance of cloth manipulation to home and industrial settings, making a general and robust robotic manipulation framework has not been fully addressed due to the the following challenges:
% Our observation is that a large subspace of these goal-conditioned tasks can be divided into two stages: 1. Unfolding, positioning, and alignment, which eliminates self-occlusion and guarantees successful downstream manipulation 2. Folding or any other fine-grain adjustments. While the first category contains acting on unstructured states and dealing with self-occlusion, the latter can be accomplished using heuristic policies or even tools such as a folding board. For this reason, we focus on the first stage in this paper: the task of taking a crumpled, self-occluded cloth and flattening it to its' 2D canonical pose at a specified position and rotation.

\begin{enumerate}

    \item \textbf{Generality}
    
    Previous works that have investigated the task of cloth folding typically rely on strong assumptions about the cloth, such as full keypoint visibility, canonicalized initial state, or a single/square cloth instance. Since clothes come in vastly different categories, shapes, and sizes, as well as unstructured and self-occluded states, these methods cannot generalize to most natural cloth configurations.
    
    \item \textbf{Precision-Efficiency Trade-off}
    
  
    Much of the existing cloth manipulation literature has been successful in using quasi-static action primitives to achieve folding, smoothing, canonicalization, and unfolding. Although single-arm quasi-static action primitives (e.g. pick and place, pick and drag) are precise and predictable, they are inefficient against crumpled and self-occluded clothes. As an alternative, recent works have shown that dynamic action primitives (e.g. flinging, blowing-air) can be extremely efficient at unfolding; however, these dynamic actions lack the precision required for more general goal-conditioned general cloth manipulation.
    
    \alper{This is sort of what I previously had, I like some of the words in it but it doesn't fit the "challenges" section but it's more like "what we need":}
      Efficient cloth manipulation requires both coarse-grained and fine-grained actions. Without large, coarse grained actions such as a fling, the task becomes difficult to solve, and self-occlusion becomes an issue. Without fine-grained actions, the model cannot quite reach the full goal(e.g. arms still stick out in random directions, corners folded in, etc.)
        
         
    \item \textbf{Large State Space and Loss of Reward Equivariances}
    
    Cloth manipulation presents a learning challenge because a single piece of cloth can deform into practically infinite configurations, not to mention that clothes come in different shapes and sizes. Prior unfolding works in cloth unfolding \cite{ha2021flingbot} \cite{huang2022mesh}, have taken advantage of equivariant reward definitions, but equivariances lose their validity in the goal-conditioned setting. Given that we want to goal-condition a cloth, the supervision must depend on both the position and the rotation of the cloth relative to the goal.
    
\end{enumerate}

To address the challenges posed above, we propose the follownig contributions:

\begin{enumerate}
  \item \textbf{Factorization of Goal Conditioning}
  
  We assert that all goal-conditioned deformable object manipulation tasks can be factorized into the \textit{deformable goal} and the \textit{rigid goal}. Abstractly, the deformable goal concerns the shape and the deformation of the cloth, and it is invariant to translations and rotations. The \textit{rigid goal} complements the deformable goal by specifying the position and the rotation of the cloth.
  
  Our work is centered around the following insights: 1. Majority useful goal-states for garments in the real world are rigid transformations of a very few deformable goals. 2. Many of these deformable goals can be achieved starting from the canonicalized deformable goal. 3. Since cloth canonicalization eliminates self-occlusion and enforces lots of structure, getting from the canonicalized state to a useful deformable goal can be achieved using demonstrations or a heuristic. 
  
  \alper{Remark: I'm not sure if we want to include this but I think it's interesting that canonicalization is 1. universal and has a clear objective 2. deals with unstructured states, whereas folding 1. has no clear objective function, it has many local optima demonstrated by a wide variety of existing folding techniques 2. requires structure. Therefore it makes more sense to \textbf{learn how to canonicalize} and \textbf{demonstrate/hardcode how to fold. }}
  
  Therefore, we demonstrate that we can accomplish category-level goal-conditioning by first training a model to canonicalize a garment category at a given rigid goal, thereby funneling all instances of that category in a structured state, and then using a simple keypoint detection model and a heuristic to fold the garment.
  
  \item  \textbf{Combinatorial Action Primitives}
  
   We propose a simple yet efficient universal multi-primitive cloth manipulation framework that unites both dynamic and quasi-static action primitives under the same reward \alper{Unification under the same reward was mentioned by Huy, is this something that's novel or worth emphasizing?}. The resulting model outperforms all single-primitive baselines in terms of both speed and performance. \alper{Is it worth highlighting that it's easy to add new primitives}
  
  \item  \textbf{Factorization Reward and Architecture}
  
  Unfolding the arm of a shirt near the goal and away from the goal must result in vastly different supervision under the rigid goal-conditioned reward; however, we can still learn from the commonality of unfolding the arm in both examples. To accomplish this, we factorize our reward into rigid and deformable components, and we similarly factorize our networks to learn each reward separately. Doing so disentangles the supervision and results in a more equivariant reward formulation. \alper{Not saying anything about the inherent value of the reward itself or the fact that it's more aligned with human preferences yet, I will confirm these things as my multi-shirt abelations conclude, what I wrote is the worst case scenario}

\end{enumerate}
%===============================================================================

==> text/method.tex <==
\section{Method}

Our method is divided into two distinct stages:

\begin{enumerate}
    \item The rigid goal-conditioned canonicalization stage, for which we train a self-supervised model inside the PyFlex cloth simulator \cite{lin2020softgym}. The goal of rigid goal-conditioned canonicalization stage is to take an arbitrarily crumpled cloth, and to execute a combination of dynamic and quasi-static actions that will canonicalize the cloth at the goal rotation and translation, ensuring keypoint visibility and satisfying the kinematic constraints for downstream tasks.
    \item A simple, user-defined follow-up folding stage parametrized by the cloth keypoints to demonstrate the viability of heuristic folding policies after RGC.
\end{enumerate}



\subsection{Action Primitive Definitions}

To achieve both efficient and precise rigid goal-conditioned canonicalization in the first stage, our approach combines Pick \& Fling and Pick \& Place primitives.

The Fling \& Place primitive is largely influenced by FlingBot \cite{ha2021flingbot} with a few modifications suited to our task.
The key difference is that our primitive is not in a fixed direction and position. The direction of the fling is determined by the rotation of the-goal, and the position of the fling depends on the translation of the rigid-goal. This ensures that we can move our model's viewport around for rigid-goal conditioning.

The Fling \& Place primitive involves a sequence of picking, lifting, stretching, and flinging actions. First, picking primitive performs a bimanual top-down grasp on the $\textbf{x}_{\text{1}}, \textbf{x}_{\text{2}}\in \mathbb{R}^3$ coordinates, which correspond to left and right grasp locations. Second, the arms lift up the cloth until there's a $5 cm$ margin with the ground, as opposed to a fixed fling height, and the height of the cloth from the ground is recorded. This is to ensure that smaller clothes do not fold back onto themselves during flinging. Third, the cloth is stretched as much as possible, with a maximum stretch width of 0.7m. Finally, the arms move forward $0.70m$ and they move linearly move down back onto the workspace surface at $1.4ms^{-1}$ by $0.70m + \frac{\text{Cloth Height}}{2}$ to ensure that the cloth is centered on the viewport.

The Pick \& Place primitive involves a sequence of picking, lifting, dragging, and placing actions. Given $\mathbf{x}_{\text{1}}, \mathbf{x}_{\text{2}} \in \mathbb{R}^3$, the cloth is top-down pinch grasped at $\mathbf{x}_{\text{1}}$, lifted by $0.1 m$, then dragged to the xy coordinate $\mathbf{x}_{\text{2}}$ and placed back down onto the board surface.

\subsection{Reward Formulation For Rigid Goal-Conditioned Canonicalization}

For each cloth instance, the goal is determined by the ground-truth canonicalized vertices of the same cloth mesh. Obtaining the canonicalized vertices is an extremely simple task, since cloth meshes in the CLOTH3D dataset, as well as many other meshes on the internet, come in a canonicalized pose. All we do is to create goal configurations is to flatten the cloth at the center of the workspace.

% Since the ground-truth vertices in simulation provide essential information for the canonicalization task, we have no way of fine-tuning our method in the real world. However, we will demonstrate later that our model can generalize quite well to the real world since the fling primitive generates lots of similar configurations to simulation.

Let the flattened two-dimensional vertices of a cloth's configuration be defined as $\{\mathbf{v}_i\}$ and the corresponding flattened goal vertices be defined as $\{ \mathbf{g}_i\}$

A naive way to define a goal is to use take the mean L2 distance of all vertices with respect to the corresponding goal vertices. Since the magnitude of this goal differs based on cloth size, we can attempt to normalize it by dividing by $\sqrt{HW}$ where $H$ and $W$ are the height and the width of the canonicalized cloth respectively. This gives us the baseline unfactorized reward:

\begin{equation}
    R_{\textrm{Unf}} = -\frac{
        \sum_i \lvert\lvert \textbf{g}_i - \textbf{v}_i\rvert\rvert
    }{\sqrt{HW}}
    \label{eq:unfactorized}
\end{equation}

Despite being a viable dense reward, L2 reward has the following deficiencies: \newline
\begin{enumerate}
    \item\textbf{Entangled supervision:} Using the naive L2 reward, adjusting the arm of a shirt at the corner of the board results in a vastly different supervision than pulling the adjusting the arm at the center of the board. How is our model supposed to learn how to adjust the arms of a shirt?
    \item\textbf{Rough reward landscape:} Actions that end up shifting most of the cloth body result in extremely sharp changes in reward, whereas smaller actions become insignificant. This makes it make to land final adjustments to the cloth.
\end{enumerate}

To address these problems, we propose the \textit{factorized reward}, which is the sum of the \textit{rigid reward}, which represents the distance of a cloth's overall translation and rotation away from a goal position, and the \textit{deformable reward}, which represents the distance of a cloth away from its canonicalized configuration in terms of shape or deformation.

To calculate the two components, we introduce a new point cloud $\{\mathbf{g'}_{i}\}$. $\{\mathbf{g'}_{i}\}$, which is obtained superimposing the goal vertices $\{\mathbf{g}_{i}\}$ onto the cloth's workspace vertices using the ICP (iterative closest point) algorithm. Note that $\{\mathbf{g'}_{i}\}$ is the combination of a planar translation and rotation of $\{\mathbf{g}_{i}\}$. Now, we define the factorized reward as follows:

\begin{align} 
    \label{eq:factorized}
    R_{\textrm{Fac}} & = (1-\alpha) R_{\textrm{Rigid}} + \alpha R_{\textrm{Deform}}
\end{align}

where the rigid cost is given by 
\begin{equation}
    R_{\textrm{Rigid}} = 
    -\frac{\sum_i \lvert\lvert \mathbf{v}_i - \mathbf{g'}_i\rvert\rvert}
    {\sqrt{HW}}
    \label{eq:rigid}
\end{equation}
and the deformable cost is given by 
\begin{equation}
    R_{\textrm{Deform}} = 
    -\frac{\sum_i \lvert\lvert \mathbf{g'}_i - \mathbf{g}_i\rvert\rvert}{
        \sqrt{HW}
    }
    \label{eq:deform}
\end{equation}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/method_reward_v1.pdf}
    \caption{\textbf{Reward Computation.} TBD: Awaiting review.}
    \label{fig:task}
\end{figure}

The first term in the sum, the deformable distance,  represents "Given that the cloth is perfectly positioned and rotated, how bad is the shape?". The second term is the rigid distance represents "If the cloth were perfectly canonicalized in place, how off would it be from one that's canonicalized at the goal?"

$\alpha$ is a tunable parameter which determines how much emphasis is put onto the deformable reward.
Our factorized architecture formulation, which we introduce in the next subsection, predicts each of these from a separate network head, so $\alpha$ can be tuned at test time to optimize a desired metric. In our experiments, we found that $\alpha=0.6$ maximizes the final IoU performance for long sleeve shirts.

\alper{I'm not sure where to properly introduce how we actually goal condition}

\subsection{Learning Reward-Maximizing Actions}

The goal of our policy is to take a top-down RGB image of the workspace, and then execute the action that will maximize the single step delta-reward that it receives. To to unify the primitive parametrizations, enforce constraints easily, and equip our model with strong inductive bias with respect to scale, translation, and rotations, we use a spatial action map approach inspired by FlingBot.


\alper{A couple sentences introducing spatial action maps}.

To extend the spatial action maps to multiple primitives, we propose a network architecture with one common encoder and $N$ decoder heads, where $N$ is the number of primitives.

For model inference, the top-down square $128 \times 128$ RGB image of the viewport is captured, concatenated with a scale invariant positional encoding, and then a batch of scaled and rotated observations are generated from this image, resulting in $B$ \textit{transformed} observations. In our experiments we use the cross product of scales $[0.75, 1.0, 1.5, 2.0, 2.5, 3.0]$ and 16 rotations spanning $360$ degrees, resulting in $B= 6 \times 16 = 96$ observations.

After a $B \times 128 \times 128$ value map is generated by each of the $N$ primitive decoders, pixels that result in an invalid action are filtered out, and the maximum value pixel among the $N \times B \times 128 \times 128$ value maps are chosen, and the chosen pixel coordinate, the chosen action primitive, and the delta rewards are recorded.


Given the pixel coordinate $(x,y)$ executed on some transformed observation, $(x,y+10)$ and $(x,y-10)$ are selected as the 2D pixel corresponding to the action primitive parameters $\mathbf{x}_1$ and $\mathbf{x}_2$. These pixel coordinates are transformed back into the world space coordinates, and the top-down depth of the coordinate is appended as the $z$ coordinate to obtain the three dimensional locations that parametrize our action primitives.

The specified action is executed, and the step statistics are saved into a replay buffer for off-policy training.

During the off-policy training stage, a batch of $(S_i, A_i, R_i)_{i=1, \cdots , N}$ tuples are sampled for each action primitive $i$, where $S_i$ represents the top-down network observation, $A_i$ represents the chosen pixel coordinate $(x, y)$, and $R_i$ represents the delta-reward received by executing the action primitive $i$ on the pixel $A_i$ with respect to the scaled and rotated reference frame of the observation $S_i$.


% \begin{algorithm}
% \caption{Multi-Primitive Off-policy Spatial Action Map}\label{alg:cap}
% \begin{algorithmic}
% \Require $n \geq 0$
% \Ensure $y = x^n$
% \State $y \gets 1$
% \State $X \gets x$
% \State $N \gets n$
% \While{$N \neq 0$}
% \If{$N$ is even}
%     \State $X \gets X \times X$
%     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% \ElsIf{$N$ is odd}
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
% \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

The loss is accumulated by sequentially forwarding each observation $S_i$ through the network, decoding the observation with the $i$ th head into a value map $V_i$, and then adding to the total loss the L2 distance between $V_i[x,y]$ and $R_i$. Once the loss is accumulated for each primitive, the gradient step is taken. In our approach, we use Adam optimizer with lr=1e-4.

In addition to predicting delta-rewards using a network, we also investigate learning rigid and deformable rewards using two separate networks, with one encoder and $N$ decoders each. For inference, the $N$ value maps from each network are added together by the weight $\alpha$ according to factorized reward formulation [\ref{eq:factorized}], and the maximum pixel is chosen for execution. The training procedure is identical to the one mentioned above, where one network is supervised on delta-rigid-rewards and the other one on delta-deformable-rewards.
For more details, we refer to readers the code [Link] %We pretend I have a well-documented code-base here%. 

We train our model using the aformentioned setup until convergence, for 12,500 episodes with 8 steps per episode. This process takes about 48 hours on 4 RTX3090 GPUs.


\subsection{Follow-up Folding Heuristic}

Unlike unfolding, folding a cloth is a structured, step-by-step task that does not involve self-occlusion. In addition, folding methods vary based on habits and preferences, so it does not make sense to train an entire model to fold a cloth in one specific way.

In our approach, we use a simple heuristic that identifies cloth keypoints using a UNet, and then executes a user-defined closed-loop policy based on these keypoints.

To train the UNet keypoint model for a given cloth category, we take about 100 128x128 pixel images of high-coverage observations from a training replay buffer, and hand-label them using a custom GUI. Using a heavily augmented training pipeline, we are able to train a model that can robustly identify the keypoints of a canonicalized cloth with high sim to real generalizability. The canonicalized pose makes the keypoint identification almost trivial.

After identifying the cloth keypoints, we execute a user-defined pick-and-place policy parametrized by the keypoint locations.


==> text/methodv2.tex <==
\section{Method}

\subsection{A Two-staged Recipe for Garment Processing}

% What is the core essence of garment manipulation
Commonly cited reasons for the challenges of cloth manipulation are their infinite degrees-of-freedom (DOF) and severely crumpled configurations, which implies a large state space and partial observability, respectively.
Thus, the same simple, low-failure-rate state machines which has dominated non-deformable manufacturing pipelines does not trivially extend to garment pipelines.
This is because such human-designed state machines typically assumes a low-dimensional state space and highly-structured configurations, which requires limited-to-no sensing.
Are we forced to take a fully end-to-end learning approach for each cloth manipulation task we care about then?

We propose to factorize a cloth-manipulation pipeline into two stages\todo{consider putting two part factorization into teaser figure}.
In the first stage, the robot system execute a learned \emph{task-agnostic} canonicalization \& alignment policy, which leaves the garment is in a standard pose with all keypoints are visible.
In the second stage, the robot will execute a \emph{task-specific} human-specified state machine, which operates purely from key-points.
We argue that this factorization comes with three benefits:
\begin{enumerate}
    \item \textbf{Arbitrary initial configuration via canonicalization}:
    Since cloths readily deform and crumple during any stage of the manufacturing pipeline, simple manually-designed state machine do not have the structure they require to perform their reliable manipulation.
    % Key-point based state machine approaches~\cite{}, such as the one we employ in the second stage, assume highly structured states -- standard configuration with all its key-points clearly visible.
    % While this ensures high key-point detection and downstream manipulation success, this is an unrealistic assumption, as cloths readily deform and crumple during any stage of the manufacturing pipeline.
    In contrast, our first stage performs canonicalization, which \emph{funnels} the large space of cloth configurations into the high-structured, fully-observable configurations which such state machines require, which enables our pipeline to work on arbitrary initial configurations.
    \item \textbf{Downstream task-awareness via alignment}:
    Manufacturing pipelines may involve many different tools (\eg iron, sewing machines) placed on different sides of a workspace.
    Thus, depending on the downstream task, it is insufficient for canonicalized cloths to be at any position and orientation on the workspace~\cite{huang2022mesh}
    In contrast, our first stage also performs garment alignment, which enables our system to canonicalize the cloth at a specified planar pose which is kinematically most suitable for downstream tasks.
    \item \textbf{Garment-level generalization via Key-point-based State Machines}:
    Engineering and debugging a task-specific state-machine operating on key-points to achieve low failure rates is much more straight forward and, thus, less costly than that for a behaviour-cloning, imitation learning, or reinforcement learning approach.
    This is because the only data-driven part of this second-stage builds upon the maturity of off-the-shelf key-point detectors and the existing user-friendly frameworks (which abstracts away the semi-supervised, data-augmentation machinery which makes them work so robustly).
    While a key-point-based cloth representation contains less information than an image~\cite{ha2021flingbot} or mesh~\cite{}, we argue that this is a feature, not a bug.
    This is because such key-point representations effectively reduces the infinite DOF down to a handful meaninful ones, which makes manually writing a state machine for a new garment manipulation task simple.
    With a good canonicalization and alignment, we hypothesize that our key-point-based state machines would achieve much better intra-garment-class generalization than data-driven approaches\todo{ideally, we have an approach which compares behaviour cloning with state machine based approaches}.
\end{enumerate}
We name our two-staged garment manufacturing pipeline recipe, which includes \underline{C}anonicalization, \underline{A}lignment, and a \underline{S}tate machine, \textbf{\OURS}.
Next, we will discuss how we formulate the canonicalization \& alignment objective (Sec.~\ref{sec:method:can_align_task}), how we learn the task (Sec.~\ref{sec:spatial_policy}), and how we implement the system and state-machines (Sec.~\ref{sec:method:heuristics}).



\subsection{The Canonicalization \& Alignment Task}
\label{sec:method:can_align_task}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/method_reward_v2.pdf}
    \caption{\textbf{Reward Computation.} TBD: Awaiting review.}
    \label{fig:task}
\end{figure}

\mypara{Problem Statement.}
Fix a garment class $c \in \{\textrm{shirt},\textrm{pants},\textrm{skirts}\}$.
Given a garment instance in class $c$ with $N$ vertices, let $\mathbf{v}= \{v_i\}_{i\in N}$ denote the local configuration of the cloth, which is the set of vertex planar positions $ v_i \in \mathbb{R}^2$ in the cloth's local frame $T = (x,y,\theta)$.
Here, $(x,y)\in \mathbb{R}^2$ is the origin and $\theta \in [-180^\circ,180^\circ]$ is the orientation of the cloth's frame with respect to the global (workspace) framework.
Denote by $ \mathbf{g}  = \{ g_i \}_{i\in N}$ the local canonical configuration of the cloth, with each $g_i \in \mathbb{R}^2$ in the cloth's local frame.
Here, $\mathbf{g}$ for each garment instance the conventional configuration for class $c$, such as the T-shaped pose when $c=\textrm{shirt}$ and the upside-down V-shaped pose $c=\textrm{pants}$.
Let the target planar pose $T^\prime = (x^\prime,y^\prime, \theta^\prime)$ describe the global planar position $(x^\prime,y^\prime) \in \mathbb{R}^2$ and rotation $\theta^\prime\in [-180^\circ,180^\circ]$ at which the garment instance's pose $T$ should be located.
Using only top-down views of the garment instance, the goal of canonicalization is to manipulate the garment instance such that  $\mathbf{v} = \mathbf{g}$.
Similarly, from only $I$, the goal of alignment is to ensure that  $T = T^\prime$.

\mypara{Naive Reward Formulation.}
Clearly, a global canonical configuration $\mathbf{g}^\prime$ can be derived from  $\mathbf{g}$ and a specified target planar pose $T^\prime$, and similarly from the current local configuration $\mathbf{v}$ to the global canonical configuration $\mathbf{v}^\prime$.
This leads to the following straight-forward objective for canonicalization and alignment
\begin{equation}
    \rewardBaseline  = -\lvert\lvert \mathbf{g}^\prime - \mathbf{v}^\prime \rvert\rvert_{2}
    \label{eq:unfactorized}
\end{equation}
By summing up the $L_2$ distances between all vertices, this objective formulation is applicable to generic cloth manipulation since $\mathbf{g}^\prime$ could be any cloth configuration of interest.
However, we argue that this leads to two downsides:
\begin{enumerate}
    \item \textbf{Entangled supervision.}
    Reaching a canonicalized configuration at the center versus the corner of the workspace could give vastly different $\rewardBaseline$ values depending on what the target planar pose $T^\prime$ is.
    This makes it difficult for the policy to tell whether it should make a planar transformation of the cloth configuration (such as shifting entire cloth to the right) or a deformable adjustment (such as flipping shirt's sleeve outwards).
    \item \textbf{Over-emphasis on cloth pose.}
    Actions that shift the cloth result in sharp and large changes in $\rewardBaseline$, while actions of smaller magnitudes become insignificant.
    Since such small adjustment actions are required to bring a poorly canonicalized cloth to a well-canonicalized one,  $\rewardBaseline$ fails to put enough emphasis on the canonicalization subtask.
\end{enumerate}

\mypara{Factorized Reward Formulation.}
In contrast, we propose a reward factorization (Fig.~\ref{fig:reward_formulation}), which retains the \underline{c}anonicalization and \underline{a}lignment nature of the task,
\begin{align} 
    \label{eq:factorized}
    \rewardOurs & = (1-\alpha) \rewardCanon + \alpha \rewardAlign
\end{align}
where $\alpha \in (0,1)$ is a weighing hyperparameter, the canonicalization reward is given by 
\begin{equation}
    \rewardCanon = 
    - \lvert\lvert \mathbf{v} - \mathbf{g}\rvert\rvert_2
    \label{eq:rigid}
\end{equation}
and the alignment reward is given by 
\begin{equation}
    \rewardAlign = 
    -\lvert\lvert \mathbf{g}^\prime - \mathbf{g}\rvert\rvert_2
    \label{eq:deform}
\end{equation}
Here, $\rewardCanon$ encodes ``if the cloth is perfectly positioned and oriented, how bad is the deformable shape?'', while $\rewardAlign$ asks, ``if the cloth was perfectly canonicalized, how bad is the planar pose offset?''.
With this factorization, we can provide separate supervision $\rewardCanon$ and $\rewardAlign$ during training, while acting with respect to $\rewardOurs$ during data-collection/inference time.
This helps the policy distinguish how actions separately affect the cloth shape or planar pose.
Further, with a tunable $\alpha$, we can emphasize $\rewardCanon$ more than $\rewardAlign$, which we have observed quantitatively correlates better with downstream task success and qualitatively aligns with a better canonicalization.

\mypara{Objective Implementation.}
In our experiments, we observed that $\alpha = 0.6$ performs best.
To account for different cloth sizes, we normalize all $\rewardCanon$, $\rewardAlign$ and $\rewardBaseline$ by the geometric mean of the cloth's height and width in a canonicalized configuration.
We define a cloth's planar pose $T$ as the planar transformation for which $\lvert\lvert\mathbf{v}^\prime - \mathbf{g}^\prime \rvert \rvert$ is minimized, and approximate this using a modified version of ICP that utilizes the ground-truth correspondence between the current mesh and the goal mesh. In this modified method, vertices that are closer to their goal coordinates below a certain threshold are used to superimpose the current vertices onto the goal vertices, and this process iterates until convergence.


\subsection{Spatial Action Maps for Canonicalization and Alignment}
\label{sec:spatial_policy}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/pipeline.png} % NOTE: exporting as png until figure is finalized, then worry about pdf figure compression afterwards
    \caption{\textbf{Approach Overview.} }
    \label{fig:pipeline}
\end{figure*}

% Why need multiple primitives, how to enable efficient learning?
Coarse-grain, high-velocity multi-arm flings can efficiently unfold and align garments from crumpled initial states~\cite{ha2021flingbot}, but is insufficient for fine-grained adjustments to achieve good canonicalization.
Instead, a multi-arm, multi-primitive system which combines quasi-static and dynamic actions can achieve the best of both worlds.
To unify the primitive parametrizations, easily enforce constraints, and equip our model with strong inductive bias with respect to scale, translation, and rotations, we use a spatial action maps policy.

% Spatial Wu_2020
\mypara{Spatial Action Maps} is a convolutional neural network~\cite{lecun2010convolutional} (CNN) based policy for learning value maps~\cite{Wu_2020} where actions are defined on the pixel grid.
% By preprocessing input images on different scales and rotations, the network becomes scale- and rotation-equivariant.
% By its CNN architecture, the network is translation-equivariant.
% Through its exploitation of these exploitation of these equivariances, spatial action maps is a popular framework for learning robotic policies~\cite{}
Through its simple and practical exploitation of these translational, rotational, and scale equivariances, spatial action maps is a popular framework for learning robotic policies~\cite{}.
We refer the reader to \citet{ha2021flingbot} for more details.

We extend \citeauthor{ha2021flingbot}'s spatial action maps approach as follows.
Given a top-down view $I\in \mathbb{R}^{H\times W \times 3}$ of the workspace (Fig.~\ref{fig:pipeline}a), we concatenate a $H \times W \times 2$ normalized coordinate map to $I$ to help the network reason about the cloth's alignment.
The resulting map is transformed to 16 rotations spanning $360^\circ$ and scales in $[0.75, 1.0, 1.5, 2.0, 2.5, 3.0]$, which effectively enforces the arm-cross-over and grasp-width safety constraints.
To enable multiple primitives, we propose a factorized network architecture (Fig.~\ref{fig:pipeline}b) with two common encoder, one for each task's reward ($\rewardCanon$, $\rewardAlign$) and multiple decoder heads, one for each primitive.
The decoded value map for each primitive from each encoder is combined using \eqref{eq:factorized}, and the highest value action (over all action parameters and primitives) is chosen (Fig.~\ref{fig:pipeline}c), with $\epsilon$-greedy exploration.

\mypara{Implementation.}
In our experiments, we consider two primitives, quasi-static pick\&place and dynamic flings.
We use $(H,W) = (128, 128)$, and a $\epsilon_v$ value exploration and $\epsilon_a$ action primitive exploration schedule with halflife $\epsilon_v=2500$ steps and $\epsilon_a=5000$ steps.
Our value networks' predictions are supervised to the delta-reward values -- which is the difference in $\rewardOurs$ before and after an action is taken -- using the MSE loss and the Adam~\cite{kingma2014adam} optimizer with a learning rate of $1e-4$.
We train our model until convergence, for 12,500 episodes with 8 optimization steps per episode, which takes about 48 hours on 4 NVIDIA RTX3090s.


\subsection{Task-specific State Machines for Ironing and Unfolding}
\label{sec:method:heuristics}

[OUTLINE]

Setup for state machines:
\begin{itemize}
    \item Run canonicalization \& alignment policy, described in previous section, with a specified target pose $T^\prime$
    \item Use DeepLabv3 to detect keypoints on the garment
    \item Execute the task-specific key-point based state machine
    \item Key benefit is that the highly structured canonicalized states enables the usage of state machines, which are simple to define and debug for engineers.
\end{itemize}

DeepLabv3
\begin{itemize}
    \item Emphasize that this is mature technology, used in many other fields, and has also been used in robotics (e.g. IRP).
    \item We collected XXX data points for each garment class, and trained one model for each garment class.
    \item Qualitatively, we observed that this key-point model generalized to novel garment instances.
    \item We provide quantitative numbers for DeepLabv3 results on held-out cloth meshes in supplementary material.
\end{itemize}

Ironing state machine for shirts:
\begin{itemize}
    \item The ironing state machine is the simplest in that it does not require any perception. A third arm holding an iron moves back and forth between two way points.
    \item Our policy performs 4 canonicalization \& alignment, one for each orientation, such that the iron covers multiple sides of the garment
    \item Ironing Score: The binary mask overlay between the iron's path and the garment.
\end{itemize}

Folding state machine for shirts:
\begin{itemize}
    \item Folding consists of 2 steps:
        \begin{enumerate}
            \item Grasp wrist keypoints, then bring them to the far waist keypoints.
            \item Grasp shoulder keypoints, then bring them to the waist keypoints.
        \end{enumerate}
    \item Folding Score: composed of three scores:
    \begin{enumerate}
        \item Shirt Body IoU score: get the shirt's body mask with the target shirt body mask, computed before step 1 of the folding state machine.
        \item Shirt Arm IoU score: similarly for shirt arms, computed between step 1 and step 2 of the folding state machine.
        \item Final folded IoU, computed after step 2 of the folding state machine.
    \end{enumerate}
    The final folding score is the mean of these three numbers.
\end{itemize}

==> text/related_work.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{example-image}
    \caption{ \textbf{Goal Conditioned Tasks.} Show task: goal conditioned task for two deformable goal, and multiple rigid goal for each deformable goal. Explain what is deformable and rigid goal }
    \label{fig:task}
\end{figure}

\section{Related work}

Prior works have explored the topics of goal-conditionining and manipulation within the domain of deformable objects. Not only are these systems limited in their manipulation capabilities (i.e. only using quasi-static or only using dynamic actions), but they also make strong assumptions about the cloth that's being manipulated (e.g. square cloth, full visibility, access to cloth image under goal configuration).   

{\color{red} I'm not sure how to group these approaches. 1 and 2 are related, but 3 and 4 are about a completely different part of the task}

\label{sec:citations}


\textbf{Reinforcement Learning for Cloth Manipulation}
\cite{wu2019withoutdemonstrations}\cite{jangir2019dynamic}
\cite{tsurumine2019deeprl}
Simplifying assumptions about square cloths or physically marked landmarks on fixed shirt dot dot dot.



\textbf{Cloth Manipulation From Expert Demonstrations} \newline
Since defining the goal by itself is a challenge in cloth manipulation, prior reinforcement learning approaches \cite{seita2019imitation, ganapathi2020learning} have leveraged expert demonstrations. While expert demonstrations simultaneously sidestep the exploration problem and the goal conditioning problem, they either rely on simplified instances such as a square cloth \cite{seita2019imitation} or expensive human input \cite{ganapathi2020learning}.


\textbf{Single Primitive Cloth Manipulation} \newline
 Bypassing the dependency on an expert, self-supervised cloth manipulation has been demonstrated in unfolding with a factorized pick \& place action space by \cite{wu2019withoutdemonstrations} and goal conditioned folding for simplified cloth instances (square cloth, rope) {\color{red} they only have unfolding btw }
 using spatial action maps~\cite{Wu_2020,zeng2019tossingbot,zeng2018learning} by \cite{lee2020learning}.
%  showed that this was also possible for the more challenging task of reaching arbitrary cloth goal states by using spatial action maps, which afforded a level of sample efficiency that made training exclusively from real-world data feasible.
However, all these approaches operate entirely in quasi-static action spaces. A recent approach \cite{ha2021flingbot} has demonstrated the effectiveness of pairing dynamic actions with spatial action maps. Although dynamic actions are useful for unfolding a cloth and reducing self-occlusion, by themselves they are not sufficient for goal-conditioned cloth manipulation. 



\textbf{Instance-level Goal Conditioning} \newline
 A learning framework developed by Hoque et. al. \cite{hoque2020robotic} first learns a cloth's visual dynamics model from random interactions, and then is able to take a visual goal image and take actions towards the goal state; however, this method assumes manipulation a square cloth. Even if visual dynamics are replaced by a more generalized framework such as optical flow \cite{weng2021fabricflownet}, which allows visual goal-conditioning on arbitrary cloth instances, it assumes that we have access to an image of a cloth in a specific goal state, which is impossible to obtain for novel cloth instances under self-occlusion.
 
 \textbf{Reward Engineering For Goal-conditioned Cloth Manipulation?}
 




% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{example-image}
%     \caption{\textbf{Pose estimation} show pose estimation (nocs) results}
%     \label{fig:task}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{example-image}
%     \caption{\textbf{Result.} walk through one example with details which action the system choose at which steps, value maps. More result with less details}
%     \label{fig:task}
% \end{figure}

